Deep Unfolding for Fast Linear Massive MIMO Precoders under a PA Consumption Model

Massive multiple-input multiple-output (MIMO) precoders are typically designed by minimizing the transmit power subject to a quality-of-service (QoS) constraint. However, current sustainability goals incentivize more energy-efficient solutions and thus it is of paramount importance to minimize the consumed power directly. Minimizing the consumed power of the power amplifier (PA), one of the most consuming components, gives rise to a convex, non-differentiable optimization problem, which has been solved in the past using conventional convex solvers. Additionally, this problem can be solved using a proximal gradient descent (PGD) algorithm, which suffers from slow convergence. In this work, to overcome the slow convergence, a deep unfolded version of the algorithm is proposed, which can achieve close-to-optimal solutions in only 20 iterations compared to the 3500 plus iterations needed by the PGD algorithm. Results indicate that the deep unfolding algorithm is three orders of magnitude faster than a conventional convex solver and four orders of magnitude faster than the PGD.

==> fig/prox_gd.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[scale=0.93]

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
xlabel shift = -5 pt,
legend cell align={left},
legend style={
nodes={scale=0.8, transform shape}, 
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204, 
    at={(0.97,0.03)},
  anchor=south east
},
tick align=outside,
tick pos=left,
xmajorgrids,
ymajorgrids,
x grid style={dotted, darkgray176},
xlabel={iterations},
ylabel={PCG},
xmin=-175, xmax=3675,
xtick style={color=black},
y grid style={dotted, darkgray176},
ymin=-0, ymax=1.18,
ytick style={color=black}
]
\addplot [semithick, black]
table {%
1 0.135074615478516
2 0.234142899513245
3 0.354238867759705
5 0.61309027671814
6 0.722752094268799
7 0.808442711830139
8 0.870935797691345
9 0.914552927017212
11 0.964213967323303
13 0.986560583114624
17 1.00138759613037
28 1.00609385967255
407 1.0278525352478
1310 1.06600916385651
2430 1.08904302120209
3500 1.09995341300964
};
\addlegendentry{\gls{pcg} - \acrfull{pgd}}
\addplot [semithick, darkorange25512714, dashed]
table {%
1 1.11602890491486
3500 1.11602890491486
};
\addlegendentry{target PCG (CVX)}
% \addplot [semithick, forestgreen4416044]
% table {%
% 1 27.3368797302246
% 2 21.9703254699707
% 3 20.7067489624023
% 4 21.8904838562012
% 5 23.950475692749
% 6 25.8162670135498
% 7 27.0421504974365
% 8 27.6669864654541
% 9 27.9037342071533
% 10 27.9428043365479
% 11 27.9014148712158
% 13 27.7776966094971
% 14 27.7279567718506
% 16 27.6617794036865
% 18 27.6271362304688
% 21 27.6047954559326
% 26 27.5949764251709
% 46 27.5928573608398
% 3500 27.5978488922119
% };
% \addlegendentry{avg sum rate}
% \addplot [semithick, crimson2143940, dotted]
% table {%
% 0 27.6754531860352
% 3499 27.6754531860352
% };
% \addlegendentry{target sum rate}
\end{axis}

\end{tikzpicture}


==> fig/speed.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[scale=0.93]
\definecolor{darkgray176}{RGB}{176,176,176}


\definecolor{blue}{HTML}{9ac7f6}
\definecolor{orange}{HTML}{ffb179}
\definecolor{green}{HTML}{60eea3}
\definecolor{jona_red}{HTML}{ff9695}
\definecolor{purple}{HTML}{d9b2ff}
\definecolor{brown}{HTML}{e4bb98}
\definecolor{pink}{HTML}{ffa4e3}
\definecolor{grey}{HTML}{cfcfcf}
\definecolor{yellow}{HTML}{fbff9f}
\definecolor{aqua}{HTML}{a7f5f2}

\begin{axis}[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.59, xmax=3.59,
xtick style={color=black},
y grid style={dotted, darkgray176},
ylabel={Time [ms]},
ymajorgrids,
ymin=0.062511451029572, ymax=3791.89213789593,
ymode=log,
ytick style={color=black},
xticklabels={_, \gls{ufpgd}-GPU, \gls{ufpgd}-CPU, CVX-CPU, \gls{pgd}-CPU},
xticklabel style = {font=\footnotesize,yshift=0.5ex}
]
\draw[draw=none,fill=blue!50] (axis cs:-0.4,0.001) rectangle (axis cs:0.4,0.103125);
\draw[draw=none,fill=aqua!50] (axis cs:0.6,0.001) rectangle (axis cs:1.4,6.434375);
\draw[draw=none,fill=orange!50] (axis cs:1.6,0.001) rectangle (axis cs:2.4,177.046875);
\draw[draw=none,fill=jona_red!50] (axis cs:2.6,0.001) rectangle (axis cs:3.4,2298.5375);
\end{axis}

\end{tikzpicture}


==> fig/unfolding_pcg.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[spy using outlines=
	{circle, magnification=2, connect spies}]

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={nodes={scale=0.8, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204,
  at={(0.97,0.03)},
  anchor=south east},
tick align=outside,
tick pos=left,
x grid style={dotted, darkgray176},
xmajorgrids,
ymajorgrids,
xlabel={iterations},
ylabel={\acrfull{pcg}},
xmin=0.0499999999999999, xmax=20.95,
xtick style={color=black},
y grid style={dotted, darkgray176},
ymin=-0.1, ymax=1.8,
ytick style={color=black}
]
\addplot [semithick, blue, mark=o, mark size=2, mark options={solid}]
table {%
1 0.0985813140869141
2 0.186825752258301
3 0.409413814544678
4 1.14461088180542
5 1.53265070915222
6 1.68553745746613
7 1.74325954914093
8 1.7552992105484
9 1.74402856826782
10 1.72036457061768
11 1.68975365161896
12 1.65518927574158
13 1.6182656288147
14 1.57970988750458
15 1.53960502147675
16 1.49740850925446
17 1.45154118537903
18 1.39716243743896
19 1.23636817932129
20 1.17011272907257
};
\addlegendentry{avg PCG - supervised \gls{ufpgd}}

\addplot [semithick, red, mark=x, mark size=2, mark options={solid}]
table {%
1 0.0894796848297119
2 0.159488320350647
3 0.307360649108887
4 0.655380725860596
5 0.937601327896118
6 1.08599162101746
7 1.14558863639832
8 1.16651916503906
9 1.17032170295715
10 1.16649389266968
11 1.15926694869995
12 1.15059590339661
13 1.14139235019684
14 1.13203012943268
15 1.1204776763916
16 1.10576450824738
17 1.09816348552704
18 1.09372591972351
19 1.09097480773926
20 1.09154069423676
};
\addlegendentry{avg PCG - unsupervised \gls{ufpgd}}

\addplot [semithick, black, mark=square, mark size=2, mark options={solid}]
table {%
1 0.135074615478516
2 0.234142899513245
3 0.354238867759705
5 0.61309027671814
6 0.722752094268799
7 0.808442711830139
8 0.870935797691345
9 0.914552927017212
10 0.944244861602783
11 0.964213967323303
13 0.986560583114624
16 0.999472737312317
20 1.00430762767792
};
\addlegendentry{avg PCG - \gls{pgd}}


\addplot [semithick, darkorange25512714, dashed]
table {%
1 1.11602890491486
20 1.11602890491486
};

\addlegendentry{target PCG (CVXPY)}

  \coordinate (spypoint) at (axis cs:19.8,1.085);
  \coordinate (magnifyglass) at (axis cs:17.5,0.725);

\end{axis}
\spy [gray, size=1.4cm] on (spypoint)
   in node[fill=white] at (magnifyglass);

\end{tikzpicture}


==> fig/unfolding_rsum.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[spy using outlines=
	{circle, magnification=3, connect spies}]

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={nodes={scale=0.8, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={dotted, darkgray176},
xlabel={iterations},
ylabel={$R{\mathrm{sum}}$ [bits/symbol]},
xmajorgrids,
ymajorgrids,
xmin=0.0499999999999999, xmax=20.95,
xtick style={color=black},
y grid style={dotted, darkgray176},
ymin=15, ymax=52.0742524130101,
ytick style={color=black}
]
\addplot [semithick, blue, mark=o, mark size= 2, mark options={solid}]
table {%
1 45.3645286560059
2 49.5992202758789
3 33.390266418457
4 19.4261894226074
5 18.3422927856445
6 18.2307281494141
7 18.2318344116211
8 18.3595523834229
9 18.5910949707031
10 18.8975410461426
11 19.2586555480957
12 19.660083770752
13 20.0935344696045
14 20.556022644043
15 21.0500183105469
16 21.5849533081055
17 22.1839065551758
18 22.9147529602051
19 25.143217086792
20 26.2268924713135
};
\addlegendentry{avg $R_{\mathrm{sum}}$ - supervised \gls{ufpgd}}
\addplot [semithick, red, mark=x, mark size= 2, mark options={solid}]
table {%
1 37.1310424804688
2 49.2663307189941
3 45.3850440979004
4 30.2811450958252
5 26.5405025482178
6 25.8368511199951
7 25.8591403961182
8 25.9797916412354
9 26.1302051544189
10 26.2946186065674
11 26.4645347595215
12 26.6340923309326
13 26.7999248504639
14 26.9612102508545
15 27.1538124084473
16 27.3936653137207
17 27.5090808868408
18 27.5722942352295
19 27.6093597412109
20 27.593391418457
};
\addlegendentry{avg $R_{\mathrm{sum}}$ - unsupervised \gls{ufpgd}}

\addplot [semithick, black, mark=square, mark size=2, mark options={solid}]
table {%
1 27.3368797302246
2 21.9703254699707
3 20.7067489624023
4 21.8904838562012
5 23.950475692749
6 25.8162670135498
7 27.0421504974365
8 27.6669864654541
9 27.9037342071533
10 27.9428043365479
11 27.9014148712158
13 27.7776966094971
14 27.7279567718506
15 27.6898593902588
16 27.6617794036865
17 27.6415386199951
19 27.6169681549072
20 27.6098155975342
};
\addlegendentry{avg $R_{\mathrm{sum}}$ - \gls{pgd}}


\addplot [semithick, darkorange25512714, dashed]
table {%
1 27.6754531860352
20 27.6754531860352
};
\addlegendentry{target $R_{\mathrm{sum}}$}

  \coordinate (spypoint) at (axis cs:20,27);
  \coordinate (magnifyglass) at (axis cs:15,35);

\end{axis}
\spy [gray, size=1.5cm] on (spypoint)
   in node[fill=white] at (magnifyglass);
   
\end{tikzpicture}

